RoboHome: Whole-Home Simulation Scene and Data Generation for Embodied Long-Horizon Loco-Manipulation

Embodied AI is moving toward long-horizon loco-manipulation and large-scale pretraining, yet such data are costly to collect on real robots, which calls for generating whole-home scenes and trajectories automatically in simulation. We present RoboHome, a whole-home simulation scene and data generation framework for embodied long-horizon loco-manipulation. Scene generation is constrained by robot loco-manipulation affordance: on real floorplans, it performs floorplan selection, room pre-layout, and joint asset-pose search, keeping assets at their original dimensions and checking robot traversal from the entrance. For data generation, a coding agent specifies the task goals and writes each task as a program, with generated videos providing human-like motion references; simulation ground truth, state rollback, and deterministic replay yield dynamically feasible long-horizon trajectories without human demonstrations. Over 60 generation attempts on 20 real floorplans, RoboHome saves a scene in 91.7% of the attempts, 28.3 and 43.3 percentage points more than Holodeck and EmbodiedGen V2; its functional completeness and layout plausibility exceed the strongest baseline by 23.9 and 22.8 points, with a collision object rate of only 0.2%. We generate data for six long-horizon tasks on the Unitree G1, the RoboParty RP1, and the wheeled dual-arm Luna. On G1, the average generation pass rate is 87.3%, authoring the expert programs costs about $70 of API fees per hour of generated data, and the generated trajectories are validated effective across multiple policy models.

==> robohome-macros.tex <==
\RequirePackage{xspace}
\RequirePackage{multirow}
\RequirePackage{makecell}

\RequirePackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\crefname{table}{Tab.}{Tabs.}
\Crefname{table}{Table}{Tables}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\newcommand{\cmark}{\ensuremath{\checkmark}}
\newcommand{\xmark}{\ensuremath{\times}}
\newcommand{\pmark}{\ensuremath{\triangle}}

\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.9}
\renewcommand{\textfraction}{0.08}
\renewcommand{\floatpagefraction}{0.7}

\setlength{\emergencystretch}{3em}

\newsavebox{\rhfitbox}
\newcommand{\fitlinewidth}[1]{%
  \sbox{\rhfitbox}{#1}%
  \ifdim\wd\rhfitbox>\linewidth
    \resizebox{\linewidth}{!}{\usebox{\rhfitbox}}%
  \else
    \usebox{\rhfitbox}%
  \fi}


==> robohome-titlepage.tex <==
\RequirePackage{fontawesome5}
\makeatletter
\newcommand{\rh@github}{}
\newcommand{\reportgithub}[1]{\renewcommand{\rh@github}{#1}}

\newcommand{\rh@icon}[1]{\makebox[1.45em][l]{\color{RPInk}#1}}
\newcommand{\rh@row}[3]{\ifdefempty{#3}{}{%
  \rh@icon{#1}\textcolor{RPMuted}{#2:}\enspace #3\par}}
\newcommand{\rh@linkrow}[3]{\ifdefempty{#3}{}{%
  \rh@icon{#1}\textcolor{RPMuted}{#2:}\enspace\expandafter\url\expandafter{#3}\par}}

\newcommand{\rh@titleseparator}{%
  \par\vspace{2mm}\noindent
  \begin{tikzpicture}
    \draw[RPBlue!25,line width=0.45pt,dash pattern=on 2pt off 2pt]
      (0,0) -- (\linewidth,0);
  \end{tikzpicture}\par\vspace{2mm}}

\renewcommand{\makereporttitle}{%
  \thispagestyle{plain}%
  \hypersetup{pdftitle={\rp@title},pdfauthor={\rp@authors},
    pdfsubject={},pdfkeywords={\rp@keywords}}%
  \begin{tcolorbox}[enhanced,breakable,colback=RPTitleBackground,
    colframe=RPTitleBackground,boxrule=0pt,arc=4mm,outer arc=4mm,
    boxsep=0pt,left=7mm,right=7mm,top=5mm,bottom=4mm,
    before skip=0pt,after skip=4mm]
  {\sffamily\bfseries\fontsize{20}{24}\selectfont\color{RPBlue}
    \raggedright\rp@title\par}
  \ifdefempty{\rp@subtitle}{}{\vspace{2mm}{\sffamily\large\color{RPMuted}
    \raggedright\rp@subtitle\par}}
  \ifdefempty{\rp@authors}{}{\vspace{3mm}{\sffamily\normalsize
    \raggedright\rp@authors\par}}
  \ifdefempty{\rp@affiliations}{}{\vspace{1mm}{\small\color{RPMuted}
    \raggedright\rp@affiliations\par}}
  \rh@titleseparator
  \noindent\begin{minipage}[c]{0.56\linewidth}
    \raggedright\sffamily\footnotesize
    \rh@row{\faCalendar[regular]}{Date}{\rp@date}
    \rh@row{\faEnvelope[regular]}{Correspondence}{\rp@contact}
    \rh@linkrow{\faGithub}{GitHub}{\rh@github}
    \rh@linkrow{\faGlobe}{Project}{\rp@projecturl}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.40\linewidth}
    \raggedleft
    \ifdefempty{\rp@logo}{\sffamily\large\bfseries\rp@headertext}{%
      \includegraphics[width=\linewidth]{\rp@logo}}
  \end{minipage}\par
  \end{tcolorbox}}
\makeatother

